FTTN: Feature-Targeted Testing for Numerical Properties of NVIDIA & AMD Matrix Accelerators

NVIDIA Tensor Cores and AMD Matrix Cores (together called Matrix Accelerators) are of growing interest in high-performance computing and machine learning owing to their high performance. Unfortunately, their numerical behaviors are not publicly documented, including the number of extra precision bits maintained, the accumulation order of addition, and predictable subnormal number handling during computations. This makes it impossible to reliably port codes across these differing accelerators. This paper contributes a collection of {\em Feature Targeted Tests for Numerical Properties} that that help determine these features across five floating-point formats, four rounding modes and additional that highlight the rounding behaviors and preservation of extra precision bits. To show the practical relevance of FTTN, we design a simple matrix-multiplication test designed with insights gathered from our feature-tests. We executed this very simple test on five platforms, producing different answers: V100, A100, and MI250X produced 0, MI100 produced 255.875, and Hopper H100 produced 191.875. Our matrix multiplication tests employ patterns found in iterative refinement-based algorithms, highlighting the need to check for significant result variability when porting code across GPUs.

==> method-logic.tex <==
There is no official document to reveal the numerical behaviors of matrix computing unit in both AMD and NVIDIA. Fasi's prior work provides the rigorous tests for NVIDIA's tensor cores, following this idea, we provide a more comprehensive tests for both AMD and NVIDIA GPUs.

\paragraph{Problem Statement}
Matrix unit is designed to compute 
$$
D = A \cot B + C
$$
To produce more accurate answer using these hardware, we want to study their numerical behaviors. Specifically, we want to study their rounding error when doing the multiplication.

The computation for each element in the final matrix is independent of each other, i.e. $D_{11} = A_{11}*B{11}+A_{12}B_{21}+...+A_{1n}B_{n1} + C_{11}$ is independent of $D_{12} = A_{11}*B{12}+A_{12}B_{22}+...+A_{1n}B_{n2} + C_{12}$, without loss of generality, we analyze the computation for one element in $D$, namely $D_{11}$, so we can just study 
$$
D_{11} = A_{11}*B{11}+A_{12}B_{21}+...+A_{1n}B_{n1} + C_{11}
$$
to conclude numerical behaviors of matrix/tensor cores. 

For this equation, 
if each number is represented exactly, then rounding error are stem from: 
\begin{enumerate}
\item Rounding error from product operation ($A_{11}*B{11}$)
\item Rounding error from accumulation operation
\end{enumerate}
Also, if the inputs are subnormal and flushed to zero when feeding into the unit, it will also cause inaccurate results. So, we can study the numerical behaviors in three aspects: 
\begin{enumerate}
    \item Are sunormal supported in both inputs and outputs.
    \item The rounding error for product (a11 * b11) 
    \item  The rounding error for accumulator (a11b11+a12b12+...annbnn + c11)
\end{enumerate}

\paragraph{Test subnormal supports}
 Testing subnormal support: Test if the matrix unit can accept subnormal input and output subnormal 
- Let a11=subnormal and a11*b11=normal number, all others as0. Check if d11 =the value a11*b11 or 0.
- Let a11 and b11 be normal number but a11*b11=subnormal number, check if d11 is subnormal or 0. 
- Let c11 be a subnormal and check if d11 is subnormal or 0. 


\paragraph{Test product operation}
 - Since the multiplication of two floating numbers with n mantissa each can result in a product with up to 2n digits in the worst case, there no precision loss for inputs fp16, tf32 (10 bits mantissa), bf16(7 bits mantissa) inputs and compute in fp32 (23 bits mantissa) precision. 
- For fp32 and fp64, 
\paragraph{Test accumulator operation}
There are several steps to test the accumulator's rounding mode and FMA features.  As mentioned in section 2.1, we need to test the extra bits used to decide the final rounding mode. To achieve this, we firstly check if one extra bit is used in a11b11+a12b12 and a11b11+c11 computation, if not used, then a simply truncate operation will be applied and the fused property will be tested directly. If one extra bit is used, then we will futhur test if this one extra bit is used in rounding or just truncate -- a breif decision of the rounding mode. Using this knowledge, we can continue test if three extra bits are used by choosing the test case that producing the different answers when using different extra bit. The rounding mode if tie and the third sticky bit will be tested if three extra bit is preserved. All these information will final tell the rounding mode of the accumlator. 

Once the rounding mode is decided, we will test the FMA property, including if only rounding and normalization once at the end, the unit width to preserve this FMA property and the the accumlation is controlled during a FMA.

1. Test if rounding at the partial sum at once at the end.
   some details
2. Test if normalzation at the partial sum or once at the end. 
   some details
3. Test the FMA preperty unit width. 
some details
4. Test if the order is controlled during one FMA unit. 
some details

\textbf{Rounding Mode Determination}
As delineated in Section~\ref{sec:fp-back}, discerning the number of extra bits used in the accumulator provides pivotal insight into its rounding behavior. So we begin our tests with assessment of the extra bits in computations.
Notice that the assessing for this part is performed by $a_{11}b_{11} + a_{12}b_{21}$ and $a_{11}b_{11} + c_{11}$. The basic rounding direction can be tested as Figure~\ref{fig:rounding} displays. Basically, $2+ulp+2*ulp$ will append `110` for the extra bis if existing. Following the principle shows in Figure~\ref{fig:guard-round-sticky}, one can decide the rounding mode by examining these two equations. However, this just gives the hints for the rounding direction. The complete rounding details need to be finished by testing the extra bit. 
\input{Figures/rounding-test}
\begin{itemize}
    \item One extra bit and the rounding direction: We can easily construct the tests to test if one extra bit existing by examining the result of $1-2*ulp$. Aligning $2*ulp$ to $1$ in binary will result in shifting the number of mantissa bit + 1, so the result will still be 1 if no extra bits are preserved. Otherwise, one extra bit is used in computation. 
    \item Rounding direction based on one extra bit: Assuring that one extra bit is used, we can test roughly the rounding direction following the tests for Figure~\ref{fig:rounding}. This information will be used to test extra three bits.  
    \item Three extra bits testing and final rounding mode. Based on the roughly rounding direction, we will conduct two tests for the three extra bits testing as the Figure~\ref{fig:3-extra-rtn} for rounding to nearest and Figure~\ref{fig:3-extra-rtz} for rounding to zero shows~\footnote{We only test these two rounding mode since they are used in matrix cores and tensor cores based on our prior tests.}. Basically, the construction idea is to align three bits when performing accumulation and make preserving one bit, two bits and three bits affect the mantissa bits differently. This can achieved by subtraction, since ... (complete it). Figure~\ref{fig:3-extra-rtn} and Figure~\ref{fig:3-extra-rtz} displays the binary computation for two numbers addition beginning with alignment.
    \input{Figures/3-extra-rtn}
    \input{Figures/3-extra-rtz}
    \item Test rounding mode for tie and sticky bit: 
\end{itemize}

\textbf{FMA Property Examination}
Upon delineating the rounding mode, our focus transitions to the accumulator's FMA attributes. Except for the FMA unit width and order controlling tests, other tests are lies on the three numbers accumulation $a_{11}b_{11} + a_{12}b_{21} + c11$ to minimize the FMA width affect. 
\begin{enumerate}
    \item \textit{Extra bits are preserved during accumulation:} This statment can be identified easily with equation $1+2^{-1}\cdot ulp + 2^{-1}\cdot ulp + 2^{-1}\cdot ulp$. If extra bits are preserved for the intermediate values, the final result should be $1+ulp$. 
    \item  \textit{Rounding once at the end:} We already know the extra bits are preserved when doing the small accumulation, that means the intermediate result will not be rounded or no reason to preserve the extra bits. 
    \item \textit{Minimum FMA unit:} For one FMA unit, the precision will be preserved during computation and rounding will perform at the last digit. That is, if addition happened not in one FMA unit, these properties won't be preserved. To test this FMA unit width, we still use the equation $1+2^{-1}\cdot ulp + 2^{-1}\cdot ulp + 2^{-1}\cdot ulp$ but shift the last $2^{-1}\cdot ulp$ along the position of the matrix multiplication as Algorithm~\ref{alg:}. As the precision of $2^{-1}\cdot ulp$ is lose as \ref{line:precision-loss}, indicating the FMA property unit is ended. 
    
    \item \textit{Normalization once at the end:} This is critical if rounding to zero and only preserve one extra bit. If normalize only once at the end, there may be one extra bit can be used for rounding when some bits are carried while doing the accumulation. On the other hand, this does no affect for extra three bits with stick bit and rounding to nearest, since this mode can already ensure round exactly. To test this property under rounding to zero and one extra case, we simply use this four numbers addition if the previous tests indicating that the minimum FMA unit is larger than four. Let $c_{11} = 1-2^{-1}\cdot ulp$, $a_{11}b_{11}=a_{12}b_{21}=2^{-2}\cdot ulp$ and $a_{13}b_{31}=ulp$. If the intermediate values are not normalized, then the precision from $2^{-2}\cdot ulp$ will be added to $1-2^{-1}\cdot ulp + a_{13}b_{31}=ulp$, resulting in  $1+ulp$.
    \input{Algorithm/min-fma-unit}
 
    \item \textit{Accumulation order is controlled in one unit:} For the FMA unit with three extra bits and rounding to nearest mode, the order is not important since all precision will be preserved. However, it may be differ if the FMA unit only preserve one extra bit and use rounding to zero mode. To test this property, we test all the permutations of equation $1+2^{-2}\cdot ulp+2^{-2}\cdot ulp+2^{-2}\cdot ulp+2^{-2}\cdot ulp$. Since only one extra bit is preserved, the precision of $2^{-2}\cdot ulp+2^{-2}\cdot ulp+2^{-2}\cdot ulp+2^{-2}\cdot ulp$ will be lose in most case except for we perform this sub-terms firstly. If the order can be controlled by assigning the values into different position inside one FMA unit, we will see one output be $1+ulp$.
\end{enumerate}
\paragraph{Testing the Product Operation}
Understanding the multiplication of floating-point numbers is pivotal. When two floating-point numbers, each with an $n$-bit mantissa, are multiplied, the resulting product can span up to $2n$ bits in its worst-case scenario.
\begin{itemize}
    \item For fp16, tf32, and bf16 Inputs: Given that these input types possess mantissas of lengths 10, 10, and 7 bits respectively, and operate in an fp32 precision with a 23-bit mantissa, no precision loss is anticipated. 
    \item 
\end{itemize}
